Distributed Multi-Agent Reinforcement Learning with One-hop Neighbors and Compute Straggler Mitigation

Most multi-agent reinforcement learning (MARL) methods are limited in the scale of problems they can handle. With increasing numbers of agents, the number of training iterations required to find the optimal behaviors increases exponentially due to the exponentially growing joint state and action spaces. This paper tackles this limitation by introducing a scalable MARL method called Distributed multi-Agent Reinforcement Learning with One-hop Neighbors (DARL1N). DARL1N is an off-policy actor-critic method that addresses the curse of dimensionality by restricting information exchanges among the agents to one-hop neighbors when representing value and policy functions. Each agent optimizes its value and policy functions over a one-hop neighborhood, significantly reducing the learning complexity, yet maintaining expressiveness by training with varying neighbor numbers and states. This structure allows us to formulate a distributed learning framework to further speed up the training procedure. Distributed computing systems, however, contain straggler compute nodes, which are slow or unresponsive due to communication bottlenecks, software or hardware problems. To mitigate the detrimental straggler effect, we introduce a novel coded distributed learning architecture, which leverages coding theory to improve the resilience of the learning system to stragglers. Comprehensive experiments show that DARL1N significantly reduces training time without sacrificing policy quality and is scalable as the number of agents increases. Moreover, the coded distributed learning architecture improves training efficiency in the presence of stragglers.

==> tex_files/background.tex <==
\section{Background}
\label{sec:background}
This section introduces the MARL problem.
%\subsection{Multi-Agent Reinforcement Learning}
In MARL, $M$ agents learn to optimize their behavior by interacting with the environment. Denote the state and action of agent $i \in [M] := \{1,\ldots,M\}$  by $s_{i}\in \mathcal{S}_i$ and $a_{i} \in \calA_i$, respectively, where $\calS_i$ and $\calA_i$ are the corresponding state and action spaces. Let $\bfs := (s_{1},\ldots, s_{M}) \in \mathcal{S} := \prod_{i \in [M]} \mathcal{S}_{i}$ and $\bfa := (a_{1}, \ldots, a_{M}) \in \mathcal{A} := \prod_{i \in [M]} \mathcal{A}_{i}$ denote the joint state and action of all agents. At time $t$, a joint action $\bfa(t)$ applied at state $\bfs(t)$ triggers a transition to a new state $\bfs(t+1) \in \calS$ according to a conditional probability density function (pdf) $p(\bfs(t+1) | \bfs(t), \bfa(t))$. After each transition, each agent $i$ receives a reward $r_i(\bfs(t),\bfa(t))$, determined by the joint state and action according to the function $r_i : \calS \times \calA \mapsto \bbR$. 
%\JX{$r_i$ already infers that the reward function can be different for different agents. This sentence can be removed.} %, where the reward functions $r_i$ may be different for different agents. 

The objective of each agent $i$ is to design a policy $\mu_i:\calS \rightarrow \calA_i$ to maximize the expected cumulative discounted reward:
%
\begin{equation}
\label{eq:value_function}
V^{\bfmu}_i(\bfs) := \mathbb{E}_{\substack{ \bfa(t)= \bfmu(\bfs(t))\\\bfs(t)\sim p\phantom{(\bfs(t))}}} \biggl[\sum_{t=0}^{\infty}\gamma^t r_i(\bfs(t),\bfa(t)) \;\big\vert\; \bfs(0)=\bfs\biggr],\nonumber
\end{equation}
%
where $\bfmu := \left(\mu_{1}, \ldots, \mu_{M}\right)$ denotes the joint policy of all agents and $\gamma \in (0,1)$ is a discount factor. The function $V^{\bfmu}_i(\bfs)$ is known as the \emph{value function} of agent $i$ associated with joint policy $\bfmu$. Many RL and MARL techniques consider stochastic policies to support the exploration-exploitation trade-off when approximating the value and policy functions \cite{RLBook}. However, since optimal policies are known to be deterministic, it is possible to directly restrict attention to deterministic policies during the learning process, e.g., as done in DDPG \cite{ddpg} and MADDPG \cite{lowe2017multi}. 

An optimal policy $\mu_i^*$ for agent $i$ can also be obtained by maximizing the \emph{action-value (Q) function}:
%
\begin{align}
\label{eq:qvalue_function}
 Q_i^{\bfmu}&(\bfs,\bfa):=\nonumber\\&  \mathbb{E}_{\substack{ \bfa(t)= \bfmu(\bfs(t))\\\bfs(t)\sim p\phantom{(\bfs(t))}}}\biggl[\sum_{t=0}^{\infty}\gamma^t r_i(\bfs(t),\bfa(t)) \;\big\vert\; \bfs(0)=\bfs, \bfa(0) = \bfa\biggr]\nonumber
\end{align}
%
and setting $\mu_i^*(\bfs) \in  \arg\max_{a_i} \max_{\bfa_{-i}} Q_i^{*}(\bfs,\bfa)$, where $Q_i^{*}(\bfs,\bfa) := \max_{\bfmu} Q_i^{\bfmu}(\bfs,\bfa)$ and $\bfa_{-i}$ denotes the actions of all agents except $i$. In the rest of the paper, we omit the time notation $t$ for simplicity, when there is no risk of confusion.






